An Efficient Algorithm for Video Super-Resolution Based On a Sequential Model

In this work, we propose a novel procedure for video super-resolution, that is the recovery of a sequence of high-resolution images from its low-resolution counterpart. Our approach is based on a "sequential" model (i.e., each high-resolution frame is supposed to be a displaced version of the preceding one) and considers the use of sparsity-enforcing priors. Both the recovery of the high-resolution images and the motion fields relating them is tackled. This leads to a large-dimensional, non-convex and non-smooth problem. We propose an algorithmic framework to address the latter. Our approach relies on fast gradient evaluation methods and modern optimization techniques for non-differentiable/non-convex problems. Unlike some other previous works, we show that there exists a provably-convergent method with a complexity linear in the problem dimensions. We assess the proposed optimization method on {several video benchmarks and emphasize its good performance with respect to the state of the art.}

==> input_soussen.tex <==
% Input file: input_soussen
%
% Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% c pour cursif : \Ac
% bb pour blackboard : \Abb
%-------------------------------------------

% DEFINITIONS PRELIMINAIRES 

\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}       % Style gras italique (necessite amsmath)           
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}} % Style gras italique (necessite amsmath)           
\def\sbv#1{\ensuremath{\mathbf{#1}}}      % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}  % Style cursif
\def\sbl#1{\ensuremath{\mathbbm{#1}}}     % Style blackboard (necessite bbm)

%-------------------------------------------

% Alphabet gras italique
\def\Ab{{\sbm{A}}\XS}  
\def\Bb{{\sbm{B}}\XS}
\def\Cb{{\sbm{C}}\XS}
\def\Ib{{\sbm{I}}\XS}  
\def\Pb{{\sbm{P}}\XS}  
\def\Xb{{\sbm{X}}\XS}  

\def\ab{{\sbm{a}}\XS}
\def\bb{{\sbm{b}}\XS} 
\def\cb{{\sbm{c}}\XS} 
\def\gb{{\sbm{g}}\XS}
\def\hb{{\sbm{h}}\XS}
\def\rb{{\sbm{r}}\XS}
\def\tb{{\sbm{t}}\XS}
\def\vb{{\sbm{v}}\XS}
\def\xb{{\sbm{x}}\XS}
\def\yb{{\sbm{y}}\XS}
\def\zb{{\sbm{z}}\XS}
\def\unb     {{\sbv{1}}\XS}

\def\alphab {{\sbmm{\alpha}}\XS}
\def\betab {{\sbmm{\beta}}\XS}
\def\Deltab {{\sbmm{\Delta}}\XS}
\def\Lambdab     {{\sbmm{\Lambda}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}

\def\zerob   {{\sbv{0}}\XS}  

% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras

\def\Ac{{\scu{A}}\XS}   
\def\Bc{{\scu{B}}\XS}   
%\def\Cc{{\scu{C}}\XS}   
\def\Nc{{\scu{N}}\XS}   
%\def\Qc{{\scu{Q}}\XS}   
%\def\Rc{{\scu{R}}\XS}   
\def\Vc{{\scu{V}}\XS}   

% Ensemble reel
\def\Rbb{{\sbl{R}}\XS}

%%%%%%%%%%%%%%%%%%% Pour definir nouvelle commande de changement de taille
\RequirePackage{ifthen}
\RequirePackage{calc}

\newcommand{\taille}[1][\scad]{%
\ifthenelse{#1 = -5}{}{}%
\ifthenelse{#1 = -4}{\tiny}{}%
\ifthenelse{#1 = -3}{\scriptsize}{}%
\ifthenelse{#1 = -2}{\footnotesize}{}%
\ifthenelse{#1 = -1}{\small}{}%
\ifthenelse{#1 = 0}{\normalsize}{}%
\ifthenelse{#1 = 1}{\large}{}%
\ifthenelse{#1 = 2}{\Large}{}%
\ifthenelse{#1 = 3}{\LARGE}{}%
\ifthenelse{#1 = 4}{\huge}{}%
\ifthenelse{#1 = 5}{\Huge}{}}

\newboolean{@serif}
\setboolean{@serif}{true}
\def\scad{-5} % scadefaultsize

\newcounter{taille}
\newcommand{\sca}[2][\scad]{\setcounter{taille}{#1}%
  \ifthenelse{\boolean{@serif}}
  {{\taille[\thetaille]\textsc{#2}}}
  {\setcounter{taille}{\value{taille}-1}{\uppercase{\taille[\thetaille]#2}}}}

% Numéro (pour biblio)
\def\numero{n°}
\def\Numero{N°}

% Liste des abreges
\def\eg{\textit{e.g.,}\XS}
\def\etal{\textit{et al.}\XS}
\def\etc{\textit{etc.}\XS}
\def\ie{\textit{i.e.,}\XS}
\def\IFF{\textit{if and only if}\XS}
\def\via{\textit{via}\XS}
\def\vs{\textit{vs}\XS}
\def\wrt{w.r.t.\XS}

% Calcul scientifique
\newcommand{\matlab}[1][\scad]{\sca[#1]{Matlab}\XS}

\newcommand{\cnrs}[1][\scad]{\sca[#1]{cnrs}\XS}

\def\CRAN{Centre de Recherche en Automatique de Nancy\XS}
\newcommand{\cran}[1][\scad]{\sca[#1]{cran, umr 7039},
   Universit\'e de Lorraine, \sca[#1]{cnrs}\XS}
\newcommand{\cranab}[1][\scad]{\sca[#1]{cran}\XS}
\newcommand{\adresseCRAN}[1][\scad]{Campus Sciences, B.P. 70239, 
F-5   4506 Vand{\oe}uvre-l\`es-Nancy, France\XS}
\newcommand{\tutelleEN}[1][\scad]{Universit\'e de Lorraine~--~\cnrs[#1]}

\def\IRCCyN{Institut de Recherche en Communication et Cybern\'etique de Nantes\XS}

%-- Accolades, parenthèses, etc --------------------------------------
        
\def\pth#1{\left(#1\right)}                \def\stdpth#1{(#1)}
\def\acc#1{\left\{#1\right\}}              \def\stdacc#1{\{#1\}}
\def\cro#1{\left[#1\right]}                \def\stdcro#1{[#1]}
\def\bars#1{\left|#1\right|}               \def\stdbars#1{|#1|}
\def\norm#1{\left\|#1\right\|}             \def\stdnorm#1{\|#1\|}
\def\scal#1{\left\langle#1\right\rangle}   \def\stdscal#1{\langle#1\rangle}
 
\def\bigpth#1{\bigl(#1\bigr)}              \def\biggpth#1{\biggl(#1\biggr)}
\def\bigacc#1{\bigl\{#1\bigr\}}            \def\biggacc#1{\biggl\{#1\biggr\}}
\def\bigcro#1{\bigl[#1\bigr]}              \def\biggcro#1{\biggl[#1\biggr]}
\def\bigbars#1{\bigl|#1\bigr|}             \def\biggbars#1{\biggl|#1\biggr|}
\def\bignorm#1{\bigl\|#1\bigr\|}           \def\biggnorm#1{\biggl\|#1\biggr\|}
\def\bigscal#1{\bigl\langle#1\bigr\rangle} \def\biggscal#1{\biggl\langle#1\biggr\rangle}

\def\Bigpth#1{\Bigl(#1\Bigr)}              \def\Biggpth#1{\Biggl(#1\Biggr)}
\def\Bigacc#1{\Bigl\{#1\Bigr\}}            \def\Biggacc#1{\Biggl\{#1\Biggr\}}
\def\Bigcro#1{\Bigl[#1\Bigr]}              \def\Biggcro#1{\Biggl[#1\Biggr]}
\def\Bigbars#1{\Bigl|#1\Bigr|}             \def\Biggbars#1{\Biggl|#1\Biggr|}
\def\Bignorm#1{\Bigl\|#1\Bigr\|}           \def\Biggnorm#1{\Biggl\|#1\Biggr\|}
\def\Bigscal#1{\Bigl\langle#1\Bigr\rangle} \def\Biggscal#1{\Biggl\langle#1\Biggr\rangle}

%-- Divers 
\def\iid{i.i.d.\XS}
\def\sgn{{\mathrm{sgn}}}

%\def\spansub#1{{\mathrm{span}}\pth{#1}}
\def\spansub#1{{\mathrm{span}}\stdpth{#1}}
\def\bigspansub#1{{\mathrm{span}}\bigpth{#1}}
\def\Card#1{{\mathrm{Card}}\cro{#1}}

\def\spark#1{{\mathrm{spark}}\stdpth{#1}}

%\def\argmax{\mathop{\mathrm{arg\,max}}} % Mieux que \def\argmax{\arg\max}
%\def\argmin{\mathop{\mathrm{arg\,min}}} % car l'indice est reparti
%
\def\froc#1#2{{#1/#2}}                  % Frac en toc


